P4SGD: Programmable Switch Enhanced Model-Parallel Training on Generalized Linear Models on Distributed FPGAs

Generalized linear models (GLMs) are a widely utilized family of machine learning models in real-world applications. As data size increases, it is essential to perform efficient distributed training for these models. However, existing systems for distributed training have a high cost for communication and often use large batch sizes to balance computation and communication, which negatively affects convergence. Therefore, we argue for an efficient distributed GLM training system that strives to achieve linear scalability, while keeping batch size reasonably low. As a start, we propose P4SGD, a distributed heterogeneous training system that efficiently trains GLMs through model parallelism between distributed FPGAs and through forward-communication-backward pipeline parallelism within an FPGA. Moreover, we propose a light-weight, latency-centric in-switch aggregation protocol to minimize the latency of the AllReduce operation between distributed FPGAs, powered by a programmable switch. As such, to our knowledge, P4SGD is the first solution that achieves almost linear scalability between distributed accelerators through model parallelism. We implement P4SGD on eight Xilinx U280 FPGAs and a Tofino P4 switch. Our experiments show P4SGD converges up to 6.5X faster than the state-of-the-art GPU counterpar.

==> context/artifact.tex <==

\section{Artifact}
 
This artifact contains all the experiments described in the "Evaluation" section of the paper. The availability of all the datasets is mentioned in the "Evaluation" section. Due to the limitation of memory capacity, we use the $amazon\_fashion$ dataset to generate a sub-dataset of 4096 samples and 332710 features to conduct experiments on this dataset, and we use the $avazu$ dataset to generate a sub-dataset of 20480 samples and 1000000 features to conduct experiments on this dataset.

\begin{enumerate}
    \item 
    \textbf{\SystemName{} Evaluation: }We run \SystemName{} on a cluster with the Wedge100BF-32X P4 reconfigurable switch and eight machines. Each machine is configured with a Intel Xeon(R) Silver 4214 CPU, and a Xilinx Alveo U280 FPGA. The source code and associated scripts are available at the Github repository https://github.com/RC4ML/P4FPGA.git. One can follow the instructions in the repo to verify the results in the paper. One needs to use the same hardware and software version.
    
    
    \item
    \textbf{GPU Baseline Evaluation: }We run GPU Baseline on a cluster with the Mellanox SN2700 switch and eight machines. Each machine is configured with a Intel Xeon(R) Silver 4214 CPU, a 100Gb/s (RDMA-enabled) Mellanox MT27800 NIC and a high-end GPU. We use 4 NVIDIA A100 and 4 NVIDIA V100. Each machine has exactly one of these GPUs. The source code and associated scripts are available at the Github repository https://github.com/RC4ML/GLMBaseline.git.
    
    \item
    \textbf{CPU Baseline Evaluation: }We run CPU Baseline on the same cluster as GPU Baseline. The source code and associated scripts are available at the Github repository https://github.com/RC4ML/GLMBaseline.git.
\end{enumerate}



$Relevant\ hardware\ details: $ Wedge100BF-32X P4 reconfigurable switch, Xilinx Alveo U280 FPGA, Mellanox SN2700 switch, Intel Xeon(R) Silver 4214 CPU, NVIDIA A100, NVIDIA V100, Mellanox MT27800 NIC

$Operating\ systems\ and\ versions:$ Ubuntu 18.04

$P4\ Compilers\ and\ versions:$ SDE-9.3.0

$FPGA\ Compilers\ and\ versions:$ Vivado 2020.1

$GPU/CPU\ Compilers\ and\ versions:$ nvcc-11.0, gcc 7.5.0, cmake-3.10.2

$Libraries\ and\ versions:$ OpenMPI v3.4.1, libnccl 2.9.6








==> context/cost_model.tex <==
\section{Cost Model}
In this section, we aim at automatically determining the optimal execution plan for distributed linear model training on FPGAs. The intuition is that adding more FPGAs might not increase the overall training performance due to inevitable long network round trip time and inherent pipeline latency. To this end, we present an analytical cost model to predict the training throughput of \SystemName{} on a pool of $F$ distributed FPGAs, each of which features $G$ engines to concurrently train on their own part of the model. 

Because each engine within an FPGA has its own HBM channels which eliminates performance interference between engines and because all engines work in lockstep, We predict the overall throughput $Th_{all}$ to be the throughput $Th$ of an engine times by the overall number ($F \times G$) of involved engines, as shown in Equation~\ref{E_throughput_overall}.
\begin{equation} \begin{scriptsize}
\label{E_throughput_overall}
\vspace{-1ex}
Th_{all} = Th \times F \times G
%\vspace{-1ex}
\end{scriptsize} \end{equation}

For each engine, the throughput $Th$ of an engine is estimated to be the minimum value between computing throughput $Th_{comp}$ and memory throughput $Th_{mem}$, as shown in Equation~\ref{E_throughput_single}.
\begin{equation} \begin{scriptsize}
\label{E_throughput_single}
\vspace{-1ex}
Th = Min (Th_{comp},Th_{mem})
%\vspace{-1ex}
\end{scriptsize} \end{equation}

% Observations: 
% 1, the networking part deeply overlaps with the computing pipeline of \SystemName, 
% 2, the role of a server is to accept the partial dot product results, aggregate these results, and broadcast the final dot product results to all the workers. 
% Therefore, the throughput is determined by all the workers. The role of each worker is to perform real linear model training and aggregate . 
% 3, all the engines on all the FPGAs work in a lock step. Therefore, the overall elapsed time is equivalent to the elapsed time of a engine. 


% where $F$ is the number of FPGAs, $G$ is the number of engines within an FPGA, $L_p$ is the fixed pipeline latency, and $L_{RTT}$ is the network round trip time for a worker from sending out a partial dot product to the server to receiving a full dot product from the server.
% \subsection{Evaluating Throughput}
% The challenge is to take the network latency ($L_{RTT}$), in terms of round trip time (RTT), into consideration. 


\subsubsection{Estimating $Th_{comp}$ for an Engine}

In this subsection, we present an analytical cost model to predict the computing throughput of an engine, which is able to consume 512 bits per cycle, so its theoretical computing throughput is 512 bits*300MB=19.2GB/s. However, the practical computing throughput should be lower, because each engine has to guarantee the RAW dependency regarding the model. There are two unavoidable factors. One factor is the pipeline latency $L$, which is distance between dot product and model updating modules. Its value is $40+2s$ cycles, where $s$ is the precision level. The other factor is the network round trip time $L_{RTT}$, whose value is 1000 cycles. \SystemName{} makes maximum possible overlap between the networking part and the computing pipeline, so $Th_{comp}$ is estimated to the theoretical computing throughput (right) multiplied by the utilization of the computing logic (left), as shown in Equation~\ref{E_computing}.

\begin{equation} \begin{scriptsize}
\label{E_computing}
\vspace{-1ex}
Th_{comp} = \cfrac{(B/8) \times \lceil M/(64*F*G)\rceil \times s}{(B/8) \times \lceil M/(64*F*G)\rceil \times s + L_p + L_{RTT}} \times 19.2, 
\vspace{-1ex}
\end{scriptsize} 
\end{equation}

%where the right part is the theoretical computing throughput and the left part is the utilization of the computing logic (i.e., dot product module). Since the chaining is enabled, the overhead of model updating can be removed. However, the pipeline latency $L_p$ cannot be ignored, especially when $M$ and $s$ are small. 


% %\noindent
% {\bf ``Wo chaining". }Now we evaluate the computing throughput of ``wo chaining", as shown in
% Equation~\ref{E_comp_wo_chaining}.
% Equation~\ref{E_comp}.
% \begin{equation} \begin{scriptsize}
% \label{E_comp_wo_chaining}
% \vspace{-1ex}
% Th_{comp} = \cfrac{(B/8) \times \lceil M/64\rceil \times s}{(1+B/8) \times \lceil M/64\rceil \times s + L} \times 25.6GB/s, 
% \vspace{-1ex}
% \end{scriptsize} \end{equation}
% where the overhead of model updating is $\lceil M/64\rceil \times s$. The dot product is idle when the model updating is active. 

\subsubsection{Estimating $Th_{mem}$ for an Engine}
MLWeaving accesses the host memory via two PCIe and one QPI links, so the memory throughput is impacted by both memory subsystem and PCIe/QPI links. This make the explicit prediction (in terms of analytical cost model) of memory throughput extremely difficult, especially under the condition the memory-related IP core on the FPGA side is encrypted. Therefore, we present an empirical cost model to evaluate the memory throughput $Th_{mem}$. 
In order to predict the memory throughput of MLWeaving, we analyze the memory access pattern of MLWeaving and then benchmark the memory throughput. % according to the memory access pattern 
Note, both ``with chaining" and ``wo chaining" have the same memory subsystem. 

{\bf Memory Access Pattern. }The memory access pattern of MLWeaving is quite fixed. Essentially, for the precision level $s$, it sequentially fetch $s$ cache lines (512 bits) every 32 cache lines, regardless of the number of features. 

{\bf Benchmarking Memory Throughput. }Based on the memory access pattern, we can benchmark the memory throughput for each precision level $s$, as shown in Equation~\ref{E_mem_bandwidth}.  
\begin{equation} \begin{scriptsize}
\label{E_mem_bandwidth}
\vspace{-1ex}
Th_{mem} = \begin{cases}
10.2GB/s &s = 1\\
13.3GB/s &s=2\\
13.8GB/s  & s=3 \\
14.8GB/s  & s\ge  4 \\
\end{cases}
\vspace{-1ex}
\end{scriptsize} \end{equation}

%Direct connection + analytical model. 


==> context/datastorage.tex <==
% \section{\StoremName{}}
% \label{dweaving}
We adapt the open-sourced MLWeaving project as our baseline data storage method. However, the baseline is not able to fully satisfy \SystemName{}’s requirement. Therefore, we improve MLWeaving in the following three aspects and present \StoremName{}. Fist, \StoremName{} stores data with any even precision. Training system with \StoremName{} can reduce a lot of memory space by choosing the precision of data. Second, Any precision of data can be chosen for calculation during training. For instance,  8 bit precision data is stored in the HBM, but you can use 3 bit precision or 4 bit precision data for training. Third, the training data read bandwidth of \StoremName{} almost reaches the maximum HBM read bandwidth which obtained in the HBM benchmark.

Compared with the memory of the CPU, the size of the HBM on the FPGA is not large. For example, the total size of the HBM on the u280 is 8 GB, the size of each HBM channel is 256 MB. We expect to make full use of the memory of HBM and choose the appropriate precision according to the size of the dataset, so we divide the data into arrays based on precision, Figure~\ref{DWeaving_layout} shows the \StoremName{} memory layout, we put bit 0, 1 in array 0, put bit 2, 3 in array 1, and $ A_{1}^{j} $ means j-th bit of feature i, sample A. However,  the throughput of memory is greatly reduced when we read a feature from different arrays, since memory read is with a large stride.


\begin{figure}
	\centering
	\includegraphics[width=3in]{figure/DWeaving_layout.png} 
	% \caption{}
	\vspace{-1ex}		
	\caption{Full-precision fixed-point memory layout converted into the \StoremName{} memory layout. As an example, we show 4-bits features} 
	%\vspace{-2.5ex}
	\label{DWeaving_layout} 
\end{figure} 



To solve the problem of low memory read efficiency with large stride, we use the work Shuhai~\cite{9114755}. Shuhai benchmark HBM on FPGAs, it presents the effect of \emph{Stride, Burst, Address Mapping Policy(AMP), etc.} on the throughput of HBM. According to Shuhai, The default AMP of HBM is "RGBCG" which has the largest throughput. The AMP of "RGBCG" means in an channel of HBM, from the 27th address bit to the 5th address bit (addr[27:5]) map to 14 bits row address, 1 bit bank group address, 2 bits bank address, 5 bits column address, 1 bit bank group address. The HBM consists of 4 bank groups where each group has 4 bank~\cite{jun2017hbm}. If we can use a different bank and bank group for each read request, then the throughput of HBM can be maximized. Figure~\ref{hbm_read} shows the different throughput from the stride to $ 2^n KB$ with the stride to $ 2^n + 1 KB$. We observe that when stride is $ 2^n + 1 KB$, each memory read request will read a different bank, the throughput of HBM can reach maximum speed. Therefore, the difference between the starting address of each array is an integer multiple of 4KB plus 1KB, so that you can ensure that the speed is the maximum when reading HBM.


% \begin{figure}
% 	\centering
% 	\subfloat[Throughput with stride to a power of 2]{\includegraphics[width=2.5in]{figure/normal_array_read.png} \label{normal_read}} 
%     %\vspace{-1ex}
%     \hfill
% 	\subfloat[Throughput with ]{\includegraphics[width=2.5in]{figure/advance_array_read.png} \label{advance_read}} 
% 	\vspace{-1ex}	
% 	\caption{Hardened 100Gb TCP stack: latency and throughput } 
% 	\vspace{-2ex}
% 	\label{hbm_read} 
% \end{figure} 



Table~\ref{memory_layout} shows an example of a \StoremName{} memory layout in HBM with engine = 2, bank = 8, feature = 512, sample = 16. 






\begin{table*}[h!]
  \centering
  \begin{scriptsize}
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \textbf{Array Index} & \textbf{Description} & \textbf{Index}& \multicolumn{3}{|c|}{\textbf{Engine0}}& ... & \multicolumn{3}{|c|}{\textbf{Engine1}}\\
    \hline
    \hline
     & & index & Bank 7 & ... & Bank 0 & ... & Bank 7 & ... & Bank 0\\
    \hline
    \multirow{8}{*}{array 0} & \multirow{2}{*}{first 32*n feature of first 8 sample} & 0 & 7 63:0 0 & ... & 0 63:0 0 & ... & 7 127:64 0 & ...  & 0 127:64 0 \\
    \cline{3-10}
    & & 1 & 7 63:0 1 & ... & 0 63:0 1 & ... & 7 127:64 1 & ... & 0 127:64 1 \\
    \cline{2-10}
    & \multirow{2}{*}{second 32*n feature of first 8 sample} & 2 & 7 191:128 0 & ... & 0 191:128 0 & ... & 7 255:192 0 & ... & 0 255:192 0 \\
    \cline{3-10}
    & & 3 & 7 191:128 1 & ... & 0 191:128 1 & ... & 7 255:192 1 & ... & 0 255:192 1 \\    
    \cline{2-10}
    & & ... & ... & ... & ... & ... & ... & ... & ... \\    
    \cline{2-10}    
    & \multirow{2}{*}{first 32*n feature of second 8 sample} & 8 & 15 63:0 0 & ... & 8 63:0 0 & ... & 15 127:64 0 & ...  & 8 127:64 0 \\
    \cline{3-10}
    & & 9 & 15 63:0 1 & ... & 8 63:0 1 & ... & 15 127:64 1 & ... & 8 127:64 1 \\    
    \cline{2-10}
    & & ... & ... & ... & ... & ... & ... & ... & ... \\ 
    \hline
    
    \multirow{8}{*}{array 1} & \multirow{2}{*}{first 32*n feature of first 8 sample} & 16 & 7 63:0 0 & ... & 0 63:0 0 & ... & 7 127:64 0 & ...  & 0 127:64 0 \\
    \cline{3-10}
    & & 17 & 7 63:0 1 & ... & 0 63:0 1 & ... & 7 127:64 1 & ... & 0 127:64 1 \\
    \cline{2-10}
    & \multirow{2}{*}{second 32*n feature of first 8 sample} & 18 & 7 191:128 0 & ... & 0 191:128 0 & ... & 7 255:192 0 & ... & 0 255:192 0 \\
    \cline{3-10}
    & & 19 & 7 191:128 1 & ... & 0 191:128 1 & ... & 7 255:192 1 & ... & 0 255:192 1 \\    
    \cline{2-10}
    & & ... & ... & ... & ... & ... & ... & ... & ... \\    
    \cline{2-10}    
    & \multirow{2}{*}{first 32*n feature of second 8 sample} & 24 & 15 63:0 0 & ... & 8 63:0 0 & ... & 15 127:64 0 & ...  & 8 127:64 0 \\
    \cline{3-10}
    & & 25 & 15 63:0 1 & ... & 8 63:0 1 & ... & 15 127:64 1 & ... & 8 127:64 1 \\    
    \cline{2-10}
    & & ... & ... & ... & ... & ... & ... & ... & ... \\ 
    \hline    
    
  \end{tabular}
  \caption{\StoremName{} memory layout u v:w x denotes the x-th bits of features(from w-th ro v-th) in the w-th sample)}
  \label{memory_layout}

\end{scriptsize}
\end{table*}



% \begin{table} [t]
% 	\centering
% 	%\begin{spacing}{0.3}
% 	%	\vspace{-1ex} 
% 	\begin{scriptsize}
% 	\caption{BWeaving memory layout: \emph{x\_y:z\_w} denotes the \emph{w}-th bits of 512 features (from $z$-th to $y$-th) in the $x$-th sample.}% and $y - z = 511$
% 	\label{t_bit_serial_instance}	
% 	\vspace{-1ex}
% 		\begin{tabular}{|p{2cm}|c||c|}
% 			\hline
% 			\textbf{Description} &\textbf{Index} & \textbf{Content ($\#CL$=512 bits)} \\%
% 			\hline
% 			\hline
% 			\hline
% 			\multirow{6}{*}{\parbox{2cm}{First 512 features of the first sample}} & $0$ & 0\_511:0\_0\\
% 			\cline{2-3}
% 			& $1$ & 0\_511:0\_1\\
% 			\cline{2-3}
% 			& $2$ & 0\_511:0\_2\\
% 			\cline{2-3}
% 			&$3$ & 0\_511:0\_3\\
% 			\cline{2-3}
% 			& $...$ & ... \\
% 			\cline{2-3}
% 			& $31$ & 0\_511:0\_31\\
% 			\hline
% 			\hline
% 			\multirow{4}{*}{\parbox{2cm}{Second 512 features of the first sample}} & $32$ & 0\_1023:512\_0\\
% 			\cline{2-3}
% 			&$33$ & 0\_1023:512\_1\\
% 			\cline{2-3}
% 			&$34$ & 0\_1023:512\_2\\
% 			\cline{2-3}
% 			&$...$ & ... \\
% 			\hline
% 			\hline
% 			$...$&$...$ & ... \\
% 			\hline
% 			\hline			\multirow{3}{*}{\parbox{2cm}{First 512 features of the second sample}} & $128$ & 1\_511:0\_0\\
% 			\cline{2-3}
% 			&$129$ & 1\_511:0\_1\\
% 			\cline{2-3}
% 			& $...$ & ... \\
% 			\hline
% 		\end{tabular}
% 	\end{scriptsize}
% 		\vspace{2ex}
% \end{table}

==> design.tex <==
\section{design}

The design of \SystemName{} includes many aspects, such as how to write data into the FPGA’s memory, how the FPGA’s computing logic is, how to transmit data through the network, how to save the model, and so on. We will discuss these designs separately.

% \subsection{Data Preparation}

% In the Intel i9-10900 + U280 platform used to implement \SystemName{}, first, we need to move the data from the main memory of the CPU to the HBM of FPGA. FPGA uses XDMA to directly access the memory of the CPU through PCIe. We have designed a $data movement$ module, which can read the data in the memory through XDMA and write it into the HBM.
% We tested the maximum speed of XDMA, which is about 12.8 GB/s, and the maximum single-channel HBM write speed is 13.2 GB/s. Therefore, in the data transfer module, we only need one write channel to write to all channels of HBM. The maximum throughput limit of PCIe can be reached.

% The computational efficiency of the training system depends on how much bit-wide data can be read per cycle. In \SystemName{}, each engine can process 512bit data per cycle, so each engine needs two HBM to read channels to read the data. Due to FPGA resource limitations, each u280 can instantiate 8 engines, so a total of 16 read channels are required. The remaining 16 channels are equally allocated to 8 engines to save sample data. Figure~\ref{hbm_to_engine} illustrates the correspondence between the channels of HBM and engines. Each engine is allocated 4 pseudo channels, 8Gb HBM memory which is used to save the dataset. During training, each engine uses two AXI interfaces to read the data in the HBM, each engine can read 512 bits of data for calculation in each cycle.

% The memory layout in HBM is based on \StoremName{} (Section~\ref{dweaving}). Each channel saves 4 banks. when training, each engine will read the data of two AXI channels at the same time, and then combine them into a bank = 8, bit = 512 data for computing.


\begin{figure}
	\centering
	\includegraphics[width=3in]{figure/hbm_engine.png} 
	% \caption{}
	\vspace{-1ex}		
	\caption{Correspondence between HBM and engine, each engine uses 4 pseudo channels} 
	%\vspace{-2.5ex}
	\label{hbm_to_engine} 
\end{figure} 



\subsection{Computing Logic}

The computing logic of \SystemName{} has many levels. A complete \SystemName{} is composed of multiple workers, and each worker is a CPU + FPGA machine. In an FPGA, the computing logic is consists of multiple engines, and in each engine, the calculation pipeline is divided into multiple banks. We introduce the whole \SystemName{} from high level to details.

\subsection{Overall Architecture of \SystemName{}}

Figure~\ref{hw_design_work} illustrates the overall architecture of \SystemName{}. \SystemName{} consists of M workers and one server. Each worker is located on an FPGA board. This FPGA board is connected to the CPU through PCIe. The CPU does not participate in the calculation process of distributed training, but only controls the \SystemName{}, displays the results, and sending the data to the memory of FPGA before the training starts.

There are N engines in each worker. After the engine calculates statistics, it sends $statistics$ to the server via 100Gb TCP stack, and waits for the server to return the sum of $statistics$, and then continues the SGD calculation.

Server is implemented on FPGA or P4 switch. there are no engines in the server, instead of an $Agg S$ module, which adds up the $statistics$ generated by all the engines in the workers and server, and sends the result to all the engines.

\begin{figure}
	\centering
	\includegraphics[width=3in]{figure/hw_design_worker.png} 
	% \caption{}
	\vspace{-1ex}		
	\caption{Overall architecture of \SystemName{}} 
	%\vspace{-2.5ex}
	\label{hw_design_work} 
\end{figure} 



\subsection{Worker Logic}

Figure~\ref{hw_design_f} illustrates the architecture of a worker. In a worker, we can choose the number of instantiated engines based on FPGA resources. A worker consists of 4 stages.

Before the training starts, the dataset is read from the memory of the CPU through PCIe in the "data movement" stage and stored in the HBM. In the next "multi-engine processing" stage, each engine corresponds to 4 pseudo channels of HBM and reads samples from it. The details of these two stages are introduced in section 5.1.

In the "statistics dispatcher" stage, the "S sender" module receives the result of the "dot product" stage in each bank and sends it to the server through the TCP stack. At the same time, the "S receiver module" receives the statistics from the server and sends them to the "gradient computation" stage in each bank.

In the "model return" stage, the entire model saved on this worker is written to the CPU memory through XDMA after each epoch training is over, and we can get the trained model from the main memory of the CPU.

\subsubsection{Engine Architecture}

Figure~\ref{hw_design_eng} presents the architecture in an engine. Each engine is a complete linear training system, and each engine saves a part of the models in ram and a part of samples in HBM. Each engine consists of 3 stages, we introduce the role of these stages.

In the “Multi-bank dividing” stage, the 512-bit input is divided into 8 banks, each of which processes 64 bit from one sample. After that, 8 banks process the 512-bit data at the same time.

In the “gradient accumulation” stage, each bank outputs 2048 bit gradient data (64 32-bit gradients), these gradients aggregate in an adder tree to get the total gradient.

In the “model update” stage, the work model which is in $model update$ is updated by the total gradient. The working model updates the 8 samples model at one cycle (corresponding to 8 banks), after a mini-batch, the $model ram$ is updated by the work model.

\subsubsection{Bank Architecture}

Figure~\ref{hw_design_b} shows the details of each bank. The goal of each bank is to process 64 bits of data per cycle. According to the distributed SGD algorithm, each bank is mainly composed of two steps. Next, we explain the details of each step.

The first stage is "dot product". There are 64 bit-serial multipliers in the "dot product" stage, and each bit-serial multiplier reads 1-bit feature data and multiply 32-bit model data in each cycle. At the same time, the feature data sent to the 64 bit-serial multipliers each cycle is stored in a 64-bit FIFO for the next "gradient computation" stage. Each bit-serial multiplier outputs a 32-bit calculation result every cycle. After that, there is an adder tree that adds up the results of the 64-bit serial multiplier. Finally, the "dot product" stage adds up the results of all the features of a sample, and then sends the result to the "S sender" module where sends the statistics to the server.

The second stage is "gradient computation". There are also 64 bit-serial multipliers at this stage. Each bit-serial multiplier reads a 1-bit feature from FIFO and multiplies it with 32-bit statistics in each cycle. Therefore, 64 bit-serial multipliers output 2048 bit gradient computation results in each cycle, and these results are output outside the bank for further processing.





\begin{figure}
	\centering
	\includegraphics[width=3in]{figure/hw_design_fpga.png} 
	% \caption{}
	\vspace{-1ex}		
	\caption{Overall architecture of each worker} 
	%\vspace{-2.5ex}
	\label{hw_design_f} 
\end{figure} 


\begin{figure}
	\centering
	\includegraphics[width=3in]{figure/hw_design_engine.png} 
	% \caption{}
	\vspace{-1ex}		
	\caption{architecture of each engine} 
	%\vspace{-2.5ex}
	\label{hw_design_eng} 
\end{figure} 

\begin{figure}
	\centering
	\includegraphics[width=3in]{figure/hw_design_bank.png} 
	% \caption{}
	\vspace{-1ex}		
	\caption{details of each bank} 
	%\vspace{-2.5ex}
	\label{hw_design_b} 
\end{figure} 


\subsection{Server Architecture}


\subsection{Optimal Design}

\subsubsection{Optimal Server}

In \SystemName{}, the function of the server is relatively simple, just aggregate the results of dot product, and it consume very few resources. If a single machine is used as a server, the performance of the machine will be wasted. So we put the worker and server on the same machine. Figure~\ref{hw_design_b} shows the architecture of the server.  

\subsubsection{Memory Layout}

\input{datastorage.tex}





\begin{figure}
	\centering
	\includegraphics[width=3in]{figure/hw_server_opt.png} 
	% \caption{}
	\vspace{-1ex}		
	\caption{details of each bank} 
	%\vspace{-2.5ex}
	\label{hw_design_b} 
\end{figure} 


\subsection{Instantiation of Hardware Design}
Talbe~\ref{t_resource_consumption} shows the resource consumption of \SystemName{} in our FPGA. The resource consumption of one engine is reasonably small. The resource utilization of one engine is less than $\%$. We instantiate 8 engines in U280, as well as other modules like PCIe, the total resource utilization is about 50$\%$.


\begin{table} [t]
	\centering
	%\begin{spacing}{0.3}
		\begin{scriptsize}
	\vspace{-0.5ex}
	\caption{Resource consumption of the hardware design for \SystemName{}}
	\label{t_resource_consumption}
	\begin{tabular}{|c||c|c|c|c|c|}
		\hline
		{\bf Hardware modules} &  {\bf LUTs} &  {\bf Registers} &  {\bf BRAMs} &  {\bf Freq.}\\
		\hline
		\hline
		{\bf PCIe} & 25824 & 34048 & 0 & 450MHz\\ 
		\hline
		{\bf TCP Stack} & 70181 & 66689 & 4.36Mb & 250MHz\\ 
		\hline
		{\bf Engine} & 1607 & 2429 & 0 & 250MHz\\ 
		\hline
		{\bf Data movement} & 672 & 1760 & 1.17Mb & 250MHz \\ 
		\hline
		{\bf Model return} & 672 & 1760 & 1.17Mb & 250MHz \\ 
		\hline		
		\hline
		{8 engines } & 104K  & 122K & 5.53Mb &  \\ %103964 122317
		\hline
		{Total resources used } & 104K  & 122K & 5.53Mb &  \\ %103964 122317
		\hline		
		{Total utilization} & 8$\%$ & 5$\%$ & 8$\%$ &  \\ %103964 122317
		\hline
	\end{tabular}
	\vspace{-2ex}

		\end{scriptsize}
	%\end{spacing}
\end{table}



==> outline.tex <==
1, abstract
2, introduction
3, background
  3.1 SGD
  3.2 P4 
  3.3 FPGA 
  3.4 Properties of Model Parallelism vs. Data Parallel in the context of hardware design

4, architecture of master-worker 
  4.1  detailed flow of model-parallel approach
     How to overlap "forward" "communication" and "backward"
  4.2  analysis of performance characteristics 
     communication latency could be the bottleneck
     propose the cost model guided approach...
     
5, system design of 
  5.1 worker
     5.1.1 multi-engine HBM
     5.1.2 
  5.2 master
     5.2.1 FPGA-based
     5.2.2 P4 based

6,  


